Localized Questions in Medical Visual Question Answering

Visual Question Answering (VQA) models aim to answer natural language questions about given images. Due to its ability to ask questions that differ from those used when training the model, medical VQA has received substantial attention in recent years. However, existing medical VQA models typically focus on answering questions that refer to an entire image rather than where the relevant content may be located in the image. Consequently, VQA models are limited in their interpretability power and the possibility to probe the model about specific image regions. This paper proposes a novel approach for medical VQA that addresses this limitation by developing a model that can answer questions about image regions while considering the context necessary to answer the questions. Our experimental results demonstrate the effectiveness of our proposed model, outperforming existing methods on three datasets. Our code and data are available at https://github.com/sergiotasconmorales/locvqa.

==> sections/material.tex <==



\begin{table}[!b]
\ra{1.1}
\begin{center}
\begin{tabular}{p{0.2cm}p{0.25\linewidth}p{0.01cm}KKKKK}
\toprule
{} &\multirow{2}{*}{Instrument}  & \multicolumn{6}{c}{Method} \\
\cmidrule{3-8} 
&         && Ignore mask & Region in Text & Crop Region & Draw Region & \ours  \\ \midrule
&Eye retractors    && \makecell[tc]{0.500 \\ $\pm$0}              & \makecell[tc]{0.822 \\ $\pm$0.005}                     & \makecell[tc]{0.882 \\ $\pm$0.002}            & \makecell[tc]{\textbf{0.913} \\$\pm$\textbf{0.002}}                 & \makecell[tc]{0.912 \\ $\pm$0.004}                        \\ 
& Rycroft cannula &&   \makecell[tc]{0.500 \\ $\pm$0}                  &   \makecell[tc]{0.728\\$\pm$0.025}                        &     \makecell[tc]{0.847\\$\pm$0.002}          &        \makecell[tc]{0.910\\$\pm$0.002}       & \makecell[tc]{\textbf{0.912}\\$\pm$\textbf{0.001}}                   \\ 
&Viter. handpiece    && \makecell[tc]{0.500 \\ $\pm$0}               & \makecell[tc]{0.805 \\$\pm$0.024}                     & \makecell[tc]{\textbf{0.960}\\$\pm$\textbf{0.006}}         & \makecell[tc]{0.953\\$\pm$0.005}              & \makecell[tc]{0.881 \\$\pm$0.010}                     \\ 
&Secondary knife &&      \makecell[tc]{0.500 \\ $\pm$0}           &   \makecell[tc]{0.751\\$\pm$0.013}       &   \makecell[tc]{0.822\\$\pm$0.013}      &  \makecell[tc]{0.828\\$\pm$0.011}       &  \makecell[tc]{\textbf{0.830}\\$\pm$\textbf{0.007}}                   \\ 

&Suture needle          && \makecell[tc]{0.500 \\ $\pm$0}                & \makecell[tc]{0.825 \\$\pm$0.019}                     & \makecell[tc]{\textbf{0.889} \\$\pm$\textbf{0.004}}         & \makecell[tc]{0.851 \\$\pm$0.014}              & \makecell[tc]{0. 848\\$\pm$0.018}    \\

&Micro-manipulator&&       \makecell[tc]{0.500 \\ $\pm$0}             &   \makecell[tc]{0.645\\$\pm$0.032}       &   \makecell[tc]{0.846\\$\pm$0.003}      &  \makecell[tc]{0.877\\$\pm$0.007}       &  \makecell[tc]{\textbf{0.889}\\$\pm$\textbf{0.004}}                   \\ 

&Bonn forceps&&       \makecell[tc]{0.500 \\ $\pm$0}              &   \makecell[tc]{0.846\\$\pm$0.020}       &   \makecell[tc]{0.908\\$\pm$0.008}      &  \makecell[tc]{0.897\\$\pm$0.012}       &  \makecell[tc]{\textbf{0.909}\\$\pm$\textbf{0.004}}                   \\ 

&Visco. cannula&&       \makecell[tc]{0.500 \\ $\pm$0}              &   \makecell[tc]{0.879\\$\pm$0.013}       &   \makecell[tc]{\textbf{0.954}\\$\pm$\textbf{0.002}}      &  \makecell[tc]{0.946\\$\pm$0.003}       &  \makecell[tc]{0.937\\$\pm$0.003}                   \\

&Cap. forceps&&       \makecell[tc]{0.500 \\ $\pm$0}              &   \makecell[tc]{0.804\\$\pm$0.039}       &   \makecell[tc]{0.905\\$\pm$0.010}      &  \makecell[tc]{\textbf{0.932}\\$\pm$\textbf{0.018}}       &  \makecell[tc]{0.908\\$\pm$0.010}                   \\

&Phaco. handpiece&&      \makecell[tc]{0.500 \\ $\pm$0}              &   \makecell[tc]{0.717\\$\pm$0.037}       &   \makecell[tc]{0.900\\$\pm$0.008}      &  \makecell[tc]{0.920\\$\pm$0.003}       &  \makecell[tc]{\textbf{0.952}\\$\pm$\textbf{0.003}}                   \\

&Charleux cannula&&       \makecell[tc]{0.500 \\ $\pm$0}              &   \makecell[tc]{0.841\\$\pm$0.044}       &   \makecell[tc]{0.826\\$\pm$0.029}      &  \makecell[tc]{0.915\\$\pm$0.016}       &  \makecell[tc]{\textbf{0.925}\\$\pm$\textbf{0.016}}                   \\

&Lens injector&&      \makecell[tc]{0.500 \\ $\pm$0}            &   \makecell[tc]{0.773\\$\pm$0.006}       &   \makecell[tc]{\textbf{0.941}\\$\pm$\textbf{0.003}}      &  \makecell[tc]{0.927\\$\pm$0.007}       &  \makecell[tc]{0.917\\$\pm$0.007}                   \\

&Cap. cystotome&&       \makecell[tc]{0.500 \\ $\pm$0}              &   \makecell[tc]{0.789\\$\pm$0.009}       &   \makecell[tc]{0.938\\$\pm$0.006}      &  \makecell[tc]{0.934\\$\pm$0.002}       &  \makecell[tc]{\textbf{0.953}\\$\pm$\textbf{0.001}}                   \\

&Primary knife&&      \makecell[tc]{0.500 \\ $\pm$0}              &   \makecell[tc]{0.846\\$\pm$0.011}       &   \makecell[tc]{\textbf{0.954}\\$\pm$\textbf{0.003}}      &  \makecell[tc]{0.926\\$\pm$0.008}       &  \makecell[tc]{0.941\\$\pm$0.0.004}                   \\

&Hydro. cannula&&       \makecell[tc]{0.500 \\ $\pm$0}               &   \makecell[tc]{0.865\\$\pm$0.006}       &   \makecell[tc]{0.939\\$\pm$0.004}          &  \makecell[tc]{\textbf{0.945}\\$\pm$\textbf{0.006}}    & \makecell[tc]{0.940\\$\pm$0.004}               \\

&A/I handpiece&&      \makecell[tc]{0.500 \\ $\pm$0}            &   \makecell[tc]{0.877\\$\pm$0.021}       &   \makecell[tc]{0.935\\$\pm$0.006}      &  \makecell[tc]{0.906\\$\pm$0.004}       &  \makecell[tc]{\textbf{0.938}\\$\pm$\textbf{0.001}}        \\           
\bottomrule
\end{tabular}
\end{center}
\caption{Average test AUC for different methods on INSEGCAT-VQA. 
}
\label{tab:results_insegcat_object}
\end{table}



\begin{figure}[]
\begin{center}
\includegraphics[width=\textwidth]{images/examples_att_supp.pdf}
\caption{Additional qualitative examples from the RIS-VQA (rows 1-3), INSEGCAT-VQA (rows 4-5) and DME-VQA (last two rows) datasets. Only the strongest baselines were considered in this comparison. The first column shows the image, the region, and the ground truth answer. Other columns show the overlaid attention maps and the answers produced by each model. Wrong answers are shown in red.}
\label{fig:examples_supp1}
\end{center}
\end{figure}
